Streaming Graph Neural Networks via Continual Learning

Graph neural networks (GNNs) have achieved strong performance in various applications. In the real world, network data is usually formed in a streaming fashion. The distributions of patterns that refer to neighborhood information of nodes may shift over time. The GNN model needs to learn the new patterns that cannot yet be captured. But learning incrementally leads to the catastrophic forgetting problem that historical knowledge is overwritten by newly learned knowledge. Therefore, it is important to train GNN model to learn new patterns and maintain existing patterns simultaneously, which few works focus on. In this paper, we propose a streaming GNN model based on continual learning so that the model is trained incrementally and up-to-date node representations can be obtained at each time step. Firstly, we design an approximation algorithm to detect new coming patterns efficiently based on information propagation. Secondly, we combine two perspectives of data replaying and model regularization for existing pattern consolidation. Specially, a hierarchy-importance sampling strategy for nodes is designed and a weighted regularization term for GNN parameters is derived, achieving greater stability and generalization of knowledge consolidation. Our model is evaluated on real and synthetic data sets and compared with multiple baselines. The results of node classification prove that our model can efficiently update model parameters and achieve comparable performance to model retraining. In addition, we also conduct a case study on the synthetic data, and carry out some specific analysis for each part of our model, illustrating its ability to learn new knowledge and maintain existing knowledge from different perspectives.

==> chapters/__latexindent_temp.tex <==
\section{Introduction}

% 网络是一种在现实世界中是非常重要的数据结构，比如社交网络、交易网络、学术网络等。网络表示学习是一种将网络节点映射到向量空间的方法，保持节点的局部信息。已有的表示学习方法可以分成两种，skip-gram模型和GNN模型，其中GNN模型深层模型，在每一层都通过聚集邻居信息来得到表示向量，从而能获得更好的效果，是目前更流行的模型。但是目前大部分方法都是针对静态网络。
Network structures are widely seen in the real world nowadays. As a method that maps nodes into vectors and preserves local structures, \textit{Network Embedding} plays an important role in many applications such as node classification and recommendation, which can be categorized in two types: SkipGram models \cite{perozzi2014deepwalk} and GNNs \cite{kipf2016semi,hamilton2017inductive}. Among them, GNNs take advantages of deep learning techniques and are capable of combining node features and local structure together, achieving great improvements than traditional models. 
But most existing methods are proposed based on the assumption that networks are static and their parameters are fixed after training. 

% 然而在真实世界中网络是不断演变的，我们得到的往往是流式的网络，比如边增加会减少，节点属性变化。网络变化后需要更新表示向量，直接在每一个时间片上重新训练复杂度高。考虑到短期内变化较少，所以没必要重新训练，而是用在线学习的方法。
% 然而网络变化导致出现一些新的模式，即从未出现过的邻域信息，而同时网网络中已有的一些模式还会存在，比如学术网络中热门邻域会随时间发生变化，比如在社交网络中不同时代的用户会有不同的朋友圈类型。因此在线学习的场景下同时保持新旧模式是重要的。
% 基于graphsage模型可以聚集邻居信息直接得到节点表示向量，但是当网络中出现新的信息时，由于模型参数是固定的，表示结果会变差。
% 但是重新训练复杂度较高。
% 流式网络下增量学习的动机：适当的对模型进行调整，即保证模型结果不会衰减，又
However, network data is usually formed in a streaming fashion and most real-world networks are continuously evolving over time, which are referred as \textit{Streaming Networks}. For example, edges are added or removed in social networks, and attributes of nodes may also change over time. Node representations need to be updated to keep fresh. A straightforward idea is to retrain GNNs once networks change but it leads to high computation complexity. Considering that networks may not change too much in a short time, an online learning method will be useful.
Furthermore, the dynamics in networks give rise to some new network distributions that have never appeared, also referred to new neighborhood patterns. In the meantime, most patterns in previous networks still maintain. For example, new research fields may grow up in citation networks and users from different ages may have distinct types of social circles.

% 相关研究，transductive的方法，在GNN上，一方面inductive不能学习新模式，另一方面online learning可能会丢失旧模式。
There are some existing researches on streaming network embedding specially, focusing on either capturing network evolutionary patterns or efficiently updating node representations. Our model belongs to the latter type, with typical examples including DANE \cite{li2017attributed} and DNE \cite{du2018dynamic}. They design strategies to update node representations in a transductive setting, which is lack of scalability and cannot be migrated to the GNN architecture. 
There are some naive incremental learning approaches for GNNs. On one hand, GNNs can efficiently generate new representations by aggregating features from neighborhood based on an inductive framework but the performance will gradually degrade as parameters do not absorb knowledge from current networks. On the other hand, applying traditional online learning approaches to GNNs cause the problem that previous patterns may be abruptly forgotten. 
Therefore, training GNNs incrementally to ensure that models are updated to learn new patterns and consolidate existing patterns simultaneously during network evolution is meaningful but few attentions have been put on it.

% 在传统的有监督学习任务中，训练数据从一个固定的分布中独立地采样，其学习目标是在最小化对于所有数据的经验损失。
% continual learning面向的是流式场景下的学习，即在真实世界中数据不会同时全部出现，不同分布、不同领域的数据以流式形式出现，不同任务中的数据$(x_i,y_i)$服从不同分布，存储所有数据并在每个时间片重新训练在大规模数据上是不可行的。continual learning的学习目标是在每一个时间片下最小化当前任务下数据的loss，而减少对之前已被学习过的数据的影响，即在数据分布发生偏移时避免灾难性遗忘问题的发生，灾难性遗忘指的是。
% 所以我们引入它解决在流式场景下GNN模型的更新问题，因为我们提到网络结构发生变化时，可能会发生分布偏移，即出现新的模式，我们GNN模型能同时学习新旧模型，同时保持较低的复杂度。
In traditional supervised learning tasks, data is sampled identically and independently from a fixed distribution $P$, and its learning goal is to minimize the empirical loss for all data. 
\textbf{Continual Learning}, also called as life-long learning, is a learning method in a streaming scenario, that is, data in the real world will not all appear at the same time. Data in different distributions and from different domains appear in a streaming manner, and data in different tasks obeys different distributions $(P^1, ..., P^T)$. Storing all data and retraining on each time step is not feasible on large-scale data. Thus, the learning goal of continual learning is to minimize the loss of data under the current task at each time step without interfering the data that has been learned before. That is when the data distribution shifts over time, it can avoid the occurrence of \textbf{catastrophic forgetting} problem that knowledge learned from previous tasks is lost as knowledge relevant to the current task is incorporated.  
Hence, we adopt continual learning to address the problem for training GNNs incrementally for the reason that network distributions may shift in streaming networks. And our goal is to develop an efficient algorithm that can not only capture new knowledge from current networks but also consolidate existing knowledge from previous networks.
% 问题挑战
% 如何捕获流式网络中的新数据。由于网络上的数据不是独立的，一个节点或者一条边的改变可能会影响到其他节点；同时发生改变并不意味着会出现新的模式。所以需要定义并设计方法找到需要进行训练的新数据。
% 如何在流式场景中保持已有模式。传统的continual learning是有task界限的，但是在流式的数据场景下这些方法不再适用。在流式场景下通过保存一个内存的节点作为整个网络的代表，来巩固已有模式的知识，但是怎么去选择并且更新这个内存中的节点是需要讨论的。
Yet, the following challenges still remain:
\begin{itemize}
    \item How to detect new patterns in streaming networks. Because nodes in networks are not independent, even changes in a small scale may influence patterns of any nodes in the entire network. Meanwhile, patterns of some changed nodes have appeared previously, which are unnecessary to be trained again. Hence, a detection algorithm should be designed for new patterns. 
    \item How to consolidate knowledge from previous networks. Traditional continual learning methods preserve old knowledge in a task-incremental setting, which cannot apply to data-incremental scenes. It remains to be discussed how to maintain and update exisitng knowledge about neighborhood patterns during network evolution.
\end{itemize}

% 技术思路。基于上述挑战，在本文中我们提出了一种针对streamingnetwork、基于continual learning的gnn框架，在网络发生变化时增量学习新增数据中包含的知识，同时巩固已有模式。
% 我们定义了流式网络中节点的受影响程度，并推导出一种基于BFS的近似计算方法，能高效地检测出网络中受影响节点。然后我们基于多角度对网络的已有知识进行建模，设计了分层-重要性的分步抽样策略，以提高数据回溯的稳定性，同时为了解决数据回溯过程的过拟合问题，进一步引入了针对模型参数的带权正则化方法。
% 针对灾难性遗忘问题，我们从数据和模型两个角度出发全面地对网络的已有知识建模，为了提高回溯数据的稳定性和优先性，我们设计了基于分层-重要性的分步抽样策略；同时我们对历史的GNN参数进行近似，推导出了在流式场景下的带权正则化方法。
% 同时，我们针对流式网络的性质，设计了对新模式的快速检测方法，和对已有模式的保存策略。我们在三个数据集上进行实验，其中两个数据集是真实的流式网络，结果证明了我们的模型远好于简单的online learning模型，同时效率远低于retraining。
Given these challenges, we propose a streaming GNN model via continual learning in streaming networks. As distributions of networks may shift over time, our model captures new patterns incrementally and consolidates existing information. 
We designed an approximation algorithm based on traversal, which can quickly detect new patterns that may exist in a streaming network. Then, based on two complementary perspectives, we propose a method to consolidate the existing knowledge in the network, that is, constraining the current model based on a small portion of historical data and the previous model.
We evaluate our model in three real-world datasets and one synthetic dataset. Our model not only obtains much better performance than naive online GNN and transductive dynamic network embedding method, but also achieves lower training time complexity than retraining models at each time step. In addition, we also conduct a case study on synthetic data, and analyze each part of the model in detail, further illustrating the model's ability to learn new knowledge and consolidate existing knowledge.

% 主要贡献
% 我们提出了一个流式GNN模型，在网络变化时高效地对模型参数进行更新，得到好的表示结果
% 我们分析了网络更新时可能发生的分布偏移的问题，并基于continuouslearning提出了我们的方法，能够同时学习新模式并保持旧模式
% 我们在真实网络上进行实验，证明了我们的模型能够同时保证效果和效率
Overall, our contributions are as follows:
\begin{itemize}
    \item We propose a streaming GNN framework that can update model parameters efficiently and generate up-to-date representations when networks evolve over time.
    \item We analyze the shifting problem of data distributions when network data is formed in a streaming fashion. A strategy based on continual learning is designed to capture new patterns and consolidate old patterns.
    \item We conduct experiments on three real-word datasets and it shows that our streaming GNNs can be updated incrementally with less accuracy lost than other models.
\end{itemize}

